Optimizing the Decoy-State BB84 QKD Protocol Parameters

The performance of a QKD implementation is determined by the tightness of the underlying security analysis. In particular, the security analyses determines the key-rate, i.e., the amount of cryptographic key material that can be distributed per time unit. Nowadays, the security analyses of various QKD protocols are well understood. It is known that optimal protocol parameters, such as the number of decoy states and their intensities, can be found by solving a nonlinear optimization problem. The complexity of this optimization problem is typically handled by making an number of heuristic assumptions. For instance, the number of decoy states is restricted to only one or two, with one of the decoy intensities set to a fixed value, and vacuum states are ignored as they are assumed to contribute only marginally to the secure key-rate. These assumptions simplify the optimization problem and reduce the size of search space significantly. However, they also cause the security analysis to be non-tight, and thereby result in sub-optimal performance. In this work, we follow a more rigorous approach using both linear and non-linear programs describing the optimization problem. Our approach, focusing on the Decoy-State BB84 protocol, allows heuristic assumptions to be omitted, and therefore results in a tighter security analysis with better protocol parameters. We show an improved performance for the Decoy-State BB84 QKD protocol, demonstrating that the heuristic assumptions typically made are too restrictive. Moreover, our improved optimization frameworks shows that the complexity of the performance optimization problem can also be handled without making heuristic assumptions, even with limited computational resources available.

==> Sections/Abstract.tex <==

\begin{abstract}
Toegevoegde waarden
\begin{itemize}
\item Inu\"itie geven waarom we dingen doen
\item Poisson verdeling afkappen goed zolang intensiteiten laag blijven $\rightarrow$ op basis van kwartielfunctie van verdeling
\item Domeinuitbreidingen
\item Intensiteiten niet rangschikken op grote, maar dit dynamisch bepalen
\item Onze krachtige optimalisatieaanpak laat zien dat sommige aannames toch wat genuanceerder zijn
\end{itemize}
\end{abstract}



==> Sections/QuantumChannel.tex <==
% !TeX root = ../main.tex
\section{Modeling the quantum channel}
\label{sec:model_quantum_channel}
In the previous section we considered the execution of the BB84 quantum key distribution protocol given a set of parameters and how to determine the key-rate for that setting using Equations~\eqref{eq:key-rate-LP}.. For Equation~\eqref{eq:keyRate_R}, we then have
\begin{equation}
R^*\left(\left(\mu_i\right)_{i\in I}, \left(p_i\right)_{i\in I}, q, n_s \right) = R^* = \frac{\ell^*}{N}
\end{equation}


The parameters optimized for this setting are By carefully choosing the parameters, this key-rate can be optimized. 

This optimisation requires the quantum channel to be modeled. 

Quantum key distribution is performed using a quantum channel. Two often used channels are free space and fiber optic cables. Independent of the used quantum channels, the theoretical analysis from the previous sections holds. Instead of actual implementations, a quantum channel can also be simulated as a model to determine the effects of particular parameter settings. Additionally, maximum key-rates can be found for given situations.  

These quantum channels can be modelled in different ways. We chose for an analytical approach and claim that this approach is beneficial over other heuristic approaches. An analytical approach is in general more complex than heuristic approximate methods, however, less assumptions are needed and improved optima can be found. 

We focus on a fiber optic quantum channel using polarization photon encoding. The analysis can easily be parsed to free space QKD or time-bin encoding. 

Photons are generated using a weak coherent laser pulse. The number of photons in each pulse is distributed by a Poisson distribution. The loss in the optic channel is exponential and the probability of photon loss at distance $x$ is given by 
\begin{equation}
%\mathbb{P}(loss\mid \text{distance } x) = 1 - e^{-\alpha x},
\eta_{channel} = 1 - e^{\alpha x},
\label{eq:channel_loss}
\end{equation}
for some attenuation factor $\alpha$. Furthermore, we denote by $\eta_{detector}$ the transmittance of the optical components in the receiver and the detector efficiency. The total loss in the quantum channel is the probability that a photon successfully arrives at the detector and is successfully detected:
\begin{equation}
\eta_{sys}=\eta_{channel}\eta_{detector}.
\end{equation}

Loss at the receiver side has two sources: the first is from misalignment of the BB84 receiver. Note that only the relative misalignment with respect to the source is relevant. Therefore, the misalignment loss at the source can be set to zero. Losses resulting from the laser source can also be set to zero by tweaking the intensities correspondingly. 

The second loss at the receiver side originates in the single photon detectors. A BB84 receiver consists of a pair of detectors for each photon state. The probability that a detector falsely registers an event, is given by the dark counts probability $p_{dark}$. This probability is fixed and the same for each detector. The yield for an $n$-photon state is the probability that this photon state causes a detection event at any of the two detectors. Losses in the detector follow either from falsely registering events (dark counts) or incorrectly registering events, which gives
\begin{equation}
Y_{n}=1-(1-p_{dark})^2(1-\eta_{sys})^n.
\end{equation}

It is standard to model attenuated laser pulses as a weak coherent laser pulse (WCP). It is assumed that global phase randomisation is applied such that WCP can be modeled as a classical mixture of Fock states. Then the number of photons emitted by each emitted pulse has a Poissonian distribution.

An often used assumption is that two extra decoy states are sufficient and the intensity of the second decoy state is near-vacuum. We instead allow for arbitrary number of decoy states.

Most other heuristic approaches only extract key-material from the one-photon pulses originating from the non-decoy intensity. We use the one-photon pulses originating from all intensities. Furthermore, we also use the zero-photon states, which still can contribute key-material due to dark-counts. 

Finally, the probability of each intensity setting is often assumed to be equal for each intensity. Also, the probability for both bases is assumed to be equal. It can be proven that for each solution with a non-uniform intensity probabilities, there is another solution at least as good, with uniform probabilities for each intensity. Therefore, the first assumption is valid. The second however, does not necessarily give an optimal key-rate and is therefore relaxed in our work.

The parameters are chosen based on parameter settings found in literature. 
\todo{This should be updated}

The security parameter are fixed as follows 
\begin{equation}
\begin{split}
\epsilon_{\text{sec}} & = 2^{-40},\\
\epsilon_{\text{cor}} & = 2^{-40},\\
p_{\text{abort}} & = 2^{-40},\\
\end{split}
\end{equation}

%The quantum channel is modeled as a configuration of optical components depicted by Fig.~\ref{fig:quantum_channel}.
%A 
%
%\begin{figure}[h]
%\centering
%trim={<left> <lower> <right> <upper>}
%\includegraphics[width=0.75\textwidth,trim={1cm 0cm 1cm 3cm},clip]{Sections/Quantum_channel.pdf}
%\caption{Quantum channel as system of optical components}
%\label{fig:quantum_channel}
%\end{figure}



